More Robust Doubly Robust Off-policy Evaluation

We study the problem of off-policy evaluation (OPE) in reinforcement learning (RL), where the goal is to estimate the performance of a policy from the data generated by another policy(ies). In particular, we focus on the doubly robust (DR) estimators that consist of an importance sampling (IS) component and a performance model, and utilize the low (or zero) bias of IS and low variance of the model at the same time. Although the accuracy of the model has a huge impact on the overall performance of DR, most of the work on using the DR estimators in OPE has been focused on improving the IS part, and not much on how to learn the model. In this paper, we propose alternative DR estimators, called more robust doubly robust (MRDR), that learn the model parameter by minimizing the variance of the DR estimator. We first present a formulation for learning the DR model in RL. We then derive formulas for the variance of the DR estimator in both contextual bandits and RL, such that their gradients w.r.t.~the model parameters can be estimated from the samples, and propose methods to efficiently minimize the variance. We prove that the MRDR estimators are strongly consistent and asymptotically optimal. Finally, we evaluate MRDR in bandits and RL benchmark problems, and compare its performance with the existing methods.

==> mdr_4.tex <==
\subsection{DM}
\label{our-DM} 

%In many applications, the expected value function model (which is a function of state and action) is approximated in a parametrized fashion. This means that for any given evaluation policy $\pi_e$, the state-action value function $Q^{\pi_e}(x,a)$ is approximated by the parameterized function $\widehat{Q}^{\pi_e}(x,a;\beta)$, where $\beta\in\RR^\kappa$ is the feature vector with dimension $\kappa\geq 0$, and  $\Phi=\{\phi(x,a)\}_{x\in\X,a\in\A}$ of state $x$ and action $a$. 
%To optimize the feature vector that minimizes the approximation error of expected reward w.r.t. policy $\pi_e$, one considers the following mean-square error minimization problem: 
%
%\begin{equation}%\label{eq:DM_opt_RL}
%\min_{\beta\in\RR^\kappa}\EE_{(x,a)\sim \rho_{\pi_e}}[(Q^{\pi_e}(x,a)-\widehat Q^{\pi_e}(x,a;\beta))^2],
%\end{equation}
%
%whose solution $\beta^*$ corresponds to the optimal value evaluation of $\pi_e$.
%Here $\rho_{\pi_e}$ is the $\gamma-$discounting state-action occupation measure induced by evaluation policy $\pi_e$, i.e., $\rho_{\pi_e}(x.a)=\frac{1-\gamma}{1-\gamma^T}\sum_{t=0}^{T-1}\gamma^t\EE_{\mu,P,\pi_e}[\mathbf 1\{x_t=x,a_t=a\}]$, where $\mathbf 1\{\cdot\}$ is an indicator function.
Since the actions in data-set $D$ is generated by the behavior policy $\pi_b$, using techniques from importance sampling, the objective function of this optimization problem can be re-written as 
$
\sum_{t=0}^{T-1}\gamma^t\EE_{\Pd}[\omega_{0:t}(\bar Q^{\pi_e}(\tau)-\widehat Q^{\pi_e}(x_t,a_t;\beta))^2]
$,
where $\bar Q^{\pi_e}(\tau)=\sum_{k=t}^{T-1}\omega_{t+1:k}\gamma^{k-t} \R(x_k,a_k)$ is an unbiased estimate of the state-action value function $ Q^{\pi_e}(x_t,a_t)$. The proof of this equivalent problem formulation is given in the appendix.
This value estimator has a bias of 
$
\EE_{\mu,\pi_e}[\Delta(x_0,a_0;\beta^*)],
$
where $\Delta(x,a;\beta)=\widehat{Q}^{\pi_e}(x, a;\beta)-Q^{\pi_e}(x,a)$ is the bias per-state-and-action pair $(x,a)\in\X\times\A$ w.r.t. model parameter $\beta$, and its variance is equal to $\frac{1}{n}\EE_{\mu}[(\EE_{\pi_e}[\Delta(x_0,a_0;\beta^*)+Q^{\pi_e}(x_0,a_0)])^2]-(\EE_{\mu,\pi_e}[\Delta(x_0,a_0;\beta^*)+Q^{\pi_e}(x_0,a_0)])^2
$.

Empirically, the objective function of the approximation error minimization problem can be further approximated by  sample-average approximation (SAA) as follows:
$\sum_{t=0}^{T-1}\gamma^t\cdot\frac{1}{n}\sum_{i=1}^n\omega^{(i)}_{0:t}(\bar Q^{\pi_e}(\tau^{(i)})-\widehat Q^{\pi_e}(x^{(i)}_t,a^{(i)}_t;\beta))^2$
where the state, action, and reward samples are from data-set $D$. Let  $\beta^*_n$ be the minimizer of the SAA minimization problem, i.e., $\beta^*_n$ satisfies the following first order optimality condition $\sum_{i=1}^n\sum_{t=0}^{T-1}\gamma^t\cdot\omega^{(i)}_{0:t}\cdot(\bar Q^{\pi_e}(\tau^{(i)})-\widehat Q^{\pi_e}(x^{(i)}_t,a^{(i)}_t;\beta))\cdot\nabla_\beta \widehat Q^{\pi_e}(x^{(i)}_t,a^{(i)}_t;\beta)=0$. 
Since the SAA estimator is unbiased, strongly consistent and asymptotically normal, when the sample size $n$ is sufficiently large, one has $\beta^*_n\rightarrow\beta^*$ almost surely. 
Followed from the relationship between a value function and a state-action value function, the value estimator w.r.t $\pi_e$ is given by 
\[
\widehat V_{DM}^{\pi_e}(\beta_n^*) =\frac{1}{n}\sum_{i=1}^n\sum_{a\in\A}\pi_e(a|x^{(i)}_0)\widehat Q^{\pi_e}(x^{(i)}_0,a;\beta^*_n).
\]
Although in practice optimizing for $\beta^*$ w.r.t. the proposed mean square error objective functions in \eqref{eq:DM_opt_RL} results in an approximate model $Q^{\pi_e}(x^{(i)}_0,a;\beta^*_n)$ that has low bias and variance, the corresponding value estimator $\widehat V_{DM}^{\pi_e}(\beta_n^*)$ is generally biased. Furthermore, there is no direct relationship between the proposed objective function and the original MSE cost function in \eqref{eq:MSE_problem}. 


==> proofs.tex <==
%!TEX root = main.tex

\subsection{Optimization Problem Formulation for Direct Method in RL}
In this section we show the equivalence of objective functions  used in the direct method. In particular, by expanding the occupation measure $\rho_{\pi_e}$ and using the change of measures by importance sampling, the following chain of equalities hold:
\[
\begin{split}
&\arg\min_{\beta\in\RR^\kappa}\EE_{(x,a)\sim \rho_{\pi_e}}\left[\left(Q^{\pi_e}(x,a)-\widehat Q^{\pi_e}(x,a;\beta)\right)^2\right]\\
=&\arg\min_{\beta\in\RR^\kappa}\sum_{t=0}^{T-1}\gamma^t\cdot\EE_{\mu,P,\pi_e}\left[\left(Q^{\pi_e}(x_t,a_t)-\widehat Q^{\pi_e}(x_t,a_t;\beta)\right)^2\right]\\
=&\arg\min_{\beta\in\RR^\kappa}\sum_{t=0}^{T-1}\gamma^t\cdot\EE_{\mu,P,\pi_e}\left[\left(\EE_{P,\pi_e}\left[\sum_{k=t}^{T-1}\gamma^{k-t} \R(x_k,a_k)\mid x_t,a_t\right]-\widehat Q^{\pi_e}(x_t,a_t;\beta)\right)^2\right]\\
=&\arg\min_{\beta\in\RR^\kappa}\sum_{t=0}^{T-1}\gamma^t\cdot\EE_{\Pd}\left[\omega_{0:t}\cdot\left(\EE_{P,\pi_b}\left[\sum_{k=t}^{T-1}\omega_{t+1:k}\cdot\gamma^{k-t} \R(x_k,a_k)\mid x_t,a_t\right]-\widehat Q^{\pi_e}(x_t,a_t;\beta)\right)^2\right]\\
=&\arg\min_{\beta\in\RR^\kappa}\sum_{t=0}^{T-1}\gamma^t\cdot\EE_{\Pd}\left[\omega_{0:t}\cdot\left(\sum_{k=t}^{T-1}\omega_{t+1:k}\cdot\gamma^{k-t} \R(x_k,a_k)-\widehat Q^{\pi_e}(x_t,a_t;\beta)\right)^2\right],
\end{split}
\]
The last equality is based on the following standard property of least square regression:
\begin{equation}\label{eq:LS_property}
\begin{split}
&\arg\min_{\beta\in\RR^\kappa}\EE_{X,Y}\left[(f(X,Y)-g(X;\beta))^2\right]\\
=&\arg\min_{\beta\in\RR^\kappa}\EE_{X,Y}\left[(f(X,Y)-\EE_{Y}[f(X,Y)|X] +\EE_{Y}[f(X,Y)|X]  - g(X;\beta))^2\right]\\
=&\arg\min_{\beta\in\RR^\kappa}\EE_{X,Y}\bigg[(f(X,Y)-\EE_{Y}[f(X,Y)|X])^2 +(\EE_{Y}[f(X,Y)|X]  - g(X;\beta))^2\\
&\quad\quad\quad\quad\quad + 2(f(X,Y)-\EE_{Y}[f(X,Y)|X])\cdot(E_{Y}[f(X,Y)|X]  - g(X;\beta))\bigg]\\
=&\arg\min_{\beta\in\RR^\kappa}\EE_{X,Y}\left[(\EE_{Y}[f(X,Y)|X]  - g(X;\beta))^2 - 2(f(X,Y)-\EE_{Y}[f(X,Y)|X])\cdot g(X;\beta)\right]\\
=&\arg\min_{\beta\in\RR^\kappa}\EE_{X,Y}\left[(\EE_{Y}[f(X,Y)|X]  - g(X;\beta))^2\right],
\end{split}
\end{equation}
where the random variables are given by: $X=(x_t,a_t)$, $Y=\{(x_{k},a_{k})\}_{k=t+1}^{T-1}$, and the cost functions are given by $f(X,Y)=\sum_{k=t}^{T-1}\omega_{t+1:k}\cdot\gamma^{k-t} \R(x_k,a_k)$, $g(X;\beta)=\widehat Q^{\pi_e}(x_t,a_t;\beta)$, for $t\in\{0,\ldots,T-1\}$. The third equality is based on the fact that the corresponding terms that are dropped are independent of $\beta$. The fourth equality is based on the fact that $\EE_{Y}[f(X,Y)-\EE_{Y}[f(X,Y)|X]\mid X]=0$.

The second part is to show that the SAA objective function is strongly consistent. Recall the SAA objective function
$
\sum_{t=0}^{T-1}\gamma^t\cdot\frac{1}{n}\sum_{i=1}^n\omega^{(i)}_{0:t}\left(\sum_{k=t}^{T-1}\omega^{(i)}_{t+1:k}\cdot\gamma^{k-t}  \,\,\R^{(i)}_k-\widehat Q^{\pi_e}\left(x^{(i)}_t,a^{(i)}_t;\beta\right)\right)^2,
$
where the state, action, and reward trajectories are from data-set $\D$ (that is generated by baseline policy $\pi_b$). This immediately implies that the SAA objective function is an unbiased sampling estimate to the original objective function: 
\[
\sum_{t=0}^{T-1}\gamma^t\cdot\EE_{\Pd}\left[\omega_{0:t}\cdot\left(\sum_{k=t}^{T-1}\omega_{t+1:k}\cdot\gamma^{k-t} \R(x_k,a_k)-\widehat Q^{\pi_e}(x_t,a_t;\beta)\right)^2\right],
\]
at each time instance $t\in\{0,\ldots,T-1\}$. Furthermore when $n\rightarrow\infty$, one has the following convergence result:
\[
\begin{split}
&\frac{1}{n}\sum_{i=1}^n\omega^{(i)}_{0:t}\cdot\left(\sum_{k=t}^{T-1}\omega^{(i)}_{t+1:k}\cdot\gamma^{k-t}  \,\,\R^{(i)}_k-\widehat Q^{\pi_e}\left(x^{(i)}_t,a^{(i)}_t;\beta\right)\right)^2\\
\rightarrow&\sum_{x_{1:T-1},a_{0:T-1}}\pi_b(a_0|x_0)\prod_{j=0}^{T-2}P(x_{j+1}|x_j,a_j)\pi_b(a_{j+1}|x_{j+1})\cdot\omega_{0:t}\cdot\left(\sum_{k=t}^{T-1}\omega_{t+1:k}\cdot\gamma^{k-t} \R(x_k,a_k)-\widehat Q^{\pi_e}(x_t,a_t;\beta)\right)^2\\
=&\EE_{\Pd}\left[\omega_{0:t}\cdot\left(\sum_{k=t}^{T-1}\omega_{t+1:k}\cdot\gamma^{k-t} \R(x_k,a_k)-\widehat Q^{\pi_e}(x_t,a_t;\beta)\right)^2\right],
\end{split}
\]
where the convergence is almost-surely (due to the assumption of the finite MDPs). This implies that the SAA objective function is strongly consistent. Furthermore, by the Central Limit Theorem, the SAA objective function is also asymptotically normal (with the mean as the original objective function). More details can be found in Section 4 of \cite{}.

